Transition Path Sampling for Rare Events in Non-Markovian Open Quantum Systems

Rare transitions govern the dynamics of many open quantum systems, but their probabilities and rates are difficult to calculate. Transition path sampling (TPS) of quantum systems has so far been limited to Markovian, perturbative descriptions. Here, we formulate TPS for non-Markovian quantum state diffusion, which is exact for Gaussian baths, extending it to non-Markovian and strongly coupled open quantum systems. For normal-to-superradiant tunneling in the unbalanced open Dicke model, we determine probabilities down to $10^{-8}$ and rates beyond the reach of brute force.

==> xrefs_letter.tex <==
\newlabel{main-FirstPage}{{}{1}{}{}{}}
\newlabel{main-eq:hamiltonian}{{1}{1}{}{}{}}
\newlabel{main-eq:bcf}{{2}{1}{}{}{}}
\newlabel{main-eq:nmqsd}{{3}{2}{}{}{}}
\newlabel{main-eq:noise_average}{{4}{2}{}{}{}}
\newlabel{main-eq:trajectory_def}{{5}{2}{}{}{}}
\newlabel{main-eq:noise_history_def}{{6}{2}{}{}{}}
\newlabel{main-fig:construction}{{1}{2}{}{}{}}
\newlabel{main-eq:pi_ab}{{7}{3}{}{}{}}
\newlabel{main-eq:acceptance}{{8}{3}{}{}{}}
\newlabel{main-eq:dicke_hamiltonian_bath}{{9}{3}{}{}{}}
\newlabel{main-eq:dicke_coupling}{{10}{3}{}{}{}}
\newlabel{main-eq:fixed_time_distribution}{{11}{3}{}{}{}}
\newlabel{main-fig:window_wham}{{2}{4}{}{}{}}
\newlabel{main-fig:rate}{{3}{4}{}{}{}}
\newlabel{main-eq:rate_final}{{12}{4}{}{}{}}
\newlabel{main-LastBibItem}{{61}{6}{}{}{}}
\newlabel{main-LastPage}{{}{6}{}{}{}}

